SoLid: A short baseline reactor neutrino experiment

The SoLid experiment, short for Search for Oscillations with a Lithium-6 detector, is a new generation neutrino experiment which tries to address the key challenges for high precision reactor neutrino measurements at very short distances from a reactor core and with little or no overburden. The primary goal of the SoLid experiment is to perform a precise measurement of the electron antineutrino energy spectrum and flux and to search for very short distance neutrino oscillations as a probe of eV-scale sterile neutrinos. This paper describes the SoLid detection principle, the mechanical design and the construction of the detector. It then reports on the installation and commissioning on site near the BR2 reactor, Belgium, and finally highlights its performance in terms of detector response and calibration.

==> 00README.XXX.tex <==
nohypertex
